Learn Fast, Forget Slow: Safe Predictive Learning Control for Systems with Unknown and Changing Dynamics Performing Repetitive Tasks

We present a control method for improved repetitive path following for a ground vehicle that is geared towards long-term operation where the operating conditions can change over time and are initially unknown. We use weighted Bayesian Linear Regression (wBLR) to model the unknown dynamics, and show how this simple model is more accurate in both its estimate of the mean behaviour and model uncertainty than Gaussian Process Regression and generalizes to novel operating conditions with little or no tuning. In addition, wBLR allows us to use fast adaptation and long-term learning in one, unified framework, to adapt quickly to new operating conditions and learn repetitive model errors over time. This comes with the added benefit of lower computational cost, longer look-ahead, and easier optimization when the model is used in a stochastic Model Predictive Controller (MPC). In order to fully capitalize on the long prediction horizons that are possible with this new approach, we use Tube MPC to reduce the growth of predicted uncertainty. We demonstrate the effectiveness of our approach in experiment on a 900\,kg ground robot showing results over 3.0\,km of driving with both physical and artificial changes to the robot's dynamics. All of our experiments are conducted using a stereo camera for localization.

==> src/conclusion.tex <==
\section{CONCLUSION}

In this paper, we have proposed a new method for long-term, safe learning control based on local, weighted BLR. This method takes advantage of the structure of the unknown dynamics to enable both fast adaptation to new scenarios and high-accuracy tracking in the presence of repetitive model errors. The model parameters can be determined reliably online which enables our method to be applied in a wide range of operating conditions with little to no tuning. We have demonstrated the effectiveness of the proposed approach in a range of challenging, off-road experiments. We encourage the reader to watch our video at \url{http://tiny.cc/fast-slow-learn} showing the experiments and datasets used in this paper.
